Modelling Gas Networks with Compressors: A port-Hamiltonian Approach

Transient gas network simulations can significantly assist in design and operational aspects of gas networks. Models used in these simulations require a detailed framework integrating various models of the network constituents - pipes and compressor stations among others. In this context, the port-Hamiltonian modelling framework provides an energy-based modelling approach with a port-based coupling mechanism. This study investigates developing compressor models in an integrated isothermal port-Hamiltonian model for gas networks. Four different models of compressors are considered and their inclusion in a larger network model is detailed. A numerical implementation for a simple testcase is provided to confirm the validity of the proposed model and to highlight their differences.

==> Makefile <==
filename?=preprint
SHELL=/bin/bash
TEX=pdflatex
FIGSTEX=pdflatex
FLAGS=-synctex=1 -interaction=nonstopmode -shell-escape
PDF=$(filename).pdf
DEPS=Makefile *.tex */*.tex *.bib *.sty
DIRS=tikz_ext
BUILD_EXTS={log,aux,out,fls,fdb_latexmk,auxlock,synctex.gz,bbl,blg,toc,bcf,run.xml,nav,snm,vrb,md5,dpth,spl}

.PHONY: all
all: $(PDF)

$(PDF): $(DEPS) | $(DIRS)
	${TEX} ${FLAGS} ${filename}
	bibtex ${filename}
	${TEX} ${FLAGS} ${filename}
	${TEX} ${FLAGS} ${filename}

figures: $(DIRS)
	@for file in tikz/*.tex; do \
		base_filename=$$(basename $$file .tex); \
		${FIGSTEX} -shell-escape -halt-on-error -interaction=batchmode \
			-jobname "tikz_ext/$${base_filename}" \
			"\def\tikzexternalrealjob{${filename}}\input{${filename}}"; \
	done

$(DIRS):
	mkdir -p $@

.PHONY: clean
clean:
	-rm -f ${filename}.${BUILD_EXTS}

.PHONY: cleanall
cleanall: clean
	-rm -rf $(DIRS)
	-rm ${filename}.pdf

.DEFAULT_GOAL = all


==> texsrc/port-Hamiltonian_systems.tex <==
\section{Port-Hamiltonian Systems}
Port-Hamiltonian systems, i.e., the combination of port-based modeling and geometric mechanics, are well suited for modeling physical networks such as gas networks. An introduction and overview can be found in~\cite{VanJ14}.
